The State of the Art in Visual Analytics for 3D Urban Data

Urbanization has amplified the importance of three-dimensional structures in urban environments for a wide range of phenomena that are of significant interest to diverse stakeholders. With the growing availability of 3D urban data, numerous studies have focused on developing visual analysis techniques tailored to the unique characteristics of urban environments. However, incorporating the third dimension into visual analytics introduces additional challenges in designing effective visual tools to tackle urban data's diverse complexities. In this paper, we present a survey on visual analytics of 3D urban data. Our work characterizes published works along three main dimensions (why, what, and how), considering use cases, analysis tasks, data, visualizations, and interactions. We provide a fine-grained categorization of published works from visualization journals and conferences, as well as from a myriad of urban domains, including urban planning, architecture, and engineering. By incorporating perspectives from both urban and visualization experts, we identify literature gaps, motivate visualization researchers to understand challenges and opportunities, and indicate future research directions.

==> 09-challenges.tex <==
\section{Research directions \& opportunities}
\label{sec:challenges}

Despite all the surveyed contributions, 3D urban visual analytics is still incipient, especially compared to its 2D counterpart.
%
In fact, the design of systems for 3D urban data analytics presents a large number of research opportunities in different areas, which we discuss next.
% Considering the myriad of domains needed to tackle urban challenges, data interoperability and the investigation of new collaborative environments are fundamental. 

% \fabio{add: (1) tailoring information to different audiences (e.g., domain experts, authorities, the general public). Specifically, the ways the information is presented (level of detail, communication medium, and usage of interaction metaphors) and the general information needs differ across these types of audiences.}

\subsection{Visual metaphors for thematic dimensions}

% Urban 3D visual analytics environments bring together many challenges 

% %
% Urban phenomena are inherently complex .
% %
% Furthermore, urban planning involve the consideration fo


While the acquisition technologies and domain analyses are becoming more sophisticated at a fast pace, the visual metaphors used to support visual analysis in 3D environments have not progressed accordingly.
%
Typical applications in urban planning involve not only studying the current state of a city but also analyzing possible scenarios for development (\emph{scenario planning}) that help business decisions and policy making.
%
In such situations, thematic dimensions are often used to visually represent the criteria used to assess the quality of the physical elements (present or future) in the city.
%
Designing visual metaphors that enable the exploration of these thematic dimensions in their spatial context is not a trivial task.
%
For example, given the complexity of cities, this can result in complex visualization scenarios such as multi-variate~\cite{doraiswamy_topology-based_2015} or temporal analysis~\cite{mota_comparison_2022}.
%
In addition, these thematic dimensions have to be explored in multiple resolutions. For example, domain experts who analyze the quality of views along the surface of a building may be interested in analyzing this quality over a high-resolution grid or by semantic elements like floors, fa\c{c}ades, or even for the entire building.
%
In such cases, visual representations that depict the distribution of aggregated values are desired~\cite{elmqvist_hierarchical_2010,srabanti_comparative_2022} but have not yet been applied in the 3D urban context.
%
\highlight{In summary, there is a pressing need for studies that design (possibly extending visual metaphors used in 2D) and evaluate visual metaphors for multi-variate and temporal data in 3D urban environments. This will enable a better support for recurring analytical scenarios in important application domains.}


Finally, the thematic dimensions used in the analysis of scenario planning are commonly the result of geometric computations or statistical modeling and, therefore, are naturally subjected to inaccuracies and uncertainty.
%
While being of great importance for spatial analysis in general~\cite{slusarski_visualisation_2019} and urban analysis in specific (\textbf{T6}), almost no attention has been given to the design of new metaphors for the visualization of uncertainty for 3D urban data.
%
Therefore, there is a need to investigate new designs to visualize uncertainty within an urban environment, as well as a more cohesive integration between urban visualization and works tackling uncertainty in information visualization~\cite{kamal_recent_2021}.
%
Another important direction is the design of visualizations that allow for the analysis of the interplay between model uncertainty and spatial context, particularly for building energy modeling, in which neighboring buildings play an important role in modeling accuracy and results~\cite{wen_fast_2022}.

There is also a need for work that provides a more grounded understanding of how different urban stakeholders (not only researchers but also policymakers) consider data uncertainties within the urban environment, and, if they do not consider it, understand their reasons~\cite{hullman_why_2020}.
%
While previous work has explored how multiple data-heavy domains deal with the different aspects of uncertainty~\cite{boukhelifa_how_2017}, no work has characterized how urban visualizations workflows are influenced by uncertainty and, especially, their propagation and impact on decision-making and policy.
%
This becomes even more pressing given the implications of the data on public policies and community participation~\cite{wan_developing_2019, dembski_digital_2019, hong_ten_2020, botin_digital_2022, wang_data_2022}.



%
% Given the many implications of 3D urban analysis on public policies and community participation~\cite{wan_developing_2019, dembski_digital_2019}, it is paramount to carefully consider the role of uncertainty
%
% Given the importance of uncertainty analysis in the urban context (\textbf{T6}) and the implications of data on public policies and community participation~\cite{wan_developing_2019, dembski_digital_2019}, 


\subsection{Data handling}

One important aspect of interactive data analytics is the fact that the latency experience from the interaction to the final visualization is important for the user experience and overall data exploration effectiveness~\cite{liu2014effects}.
%
For this reason, a large number of works have devoted attention to designing data handling strategies to support interactive exploration of large datasets~\cite{doraiswamy_interactive_2018,battle2021structured}.
%
In particular, a large body of this work was designed to support the exploration of spatiotemporal data, where the spatial component is 2D.
%
These strategies support operations such as filtering and hierarchical aggregation of thematic data for large datasets.
%
However, these solutions have not been extended to 3D spatial data.
%
For this reason, current 3D urban analytics systems use ad hoc data handling solutions, which often limit their data exploration capabilities and/or their performance.
%
With the increase in data availability, there is a strong need for solutions that could support interactive explorations of 3D urban data.
%
In particular, such a solution has to be expressive to allow for queries that align with the semantic elements in a city: buildings, fa\c{c}ades, floors, windows, streets, neighborhoods, etc. 
%
Also, it has to be efficient to support the interactive navigation, filtering, and change in the aggregation of the data.
Furthermore, this solution needs to allow for the generation and indexing of varied thematic dimensions, which is of great importance for scenario planning~\cite{ferreira_urbane_2015,doraiswamy_topology-based_2015}.

\subsection{Guided explorations and navigation}

As the scale of data grows (larger spatial coverage and/or higher resolution), there is a need for innovative mechanisms to guide data exploration and visualization, with a particular emphasis on accommodating the complexities of 3D interactions.
%
% new data exploration guidance mechanisms \& visualizations are going to be needed, specifically taking into account the burden of 3D interactions.
%
This is especially true when considering more complex scenarios such as temporal or multi-variate thematic data and highly occluded dense environments (e.g., large urban centers).
%
In these cases, interesting urban patterns can happen in multiple (spatial/temporal) scales, and the process of searching through it by basic pan, zoom, and filtering can be ineffective.
%
To help with this issue, methods that help users automatically or semi-automatically suggest points of view or data slices to inspect, can be effective in helping users to find interesting patterns.
%
In the case of 2D maps, there have been several techniques that help users to target specific portions of the thematic data, i.e., help to locate interesting points in space and time for further inspection. 
%
For example, the techniques proposed by Doraiswamy et al.~\cite{doraiswamy_using_2014}, Valdivia et al.~\cite{valdivia_wavelet-based_2015}, and Liu et al.~\cite{liu_tpflow_2019} perform spatiotemporal pattern mining based on computational topology, graph signal processing, and tensor decomposition, respectively. In the context of scientific visualization, multiple works have proposed approaches to facilitate the exploration of volumetric data~\cite{beyer_connectomeexplorer_2013,gu_mining_2016,pandey_cerebrovis_2020}. Ortner et al.~\cite{ortner2016visual} propose a methodological framework on the integration of 3D spatial and non-spatial visualizations. However, they do not offer concrete implementations tailored to 3D urban geometry nor the integration of temporal data. 
%
Such techniques have not been applied in the context of 3D urban visualization systems. 
%
One important aspect to notice is that their computational costs and their integration with the other elements in the visual interface of a system present significant challenges.

Automated techniques exist to solve the related problems of disocclusion~\cite{deng_interactive_2016}, viewpoint management, and route design~\cite{neuville_3d_2019}.
%
However, these techniques try to select the best viewpoints of a target object once this object is identified.
%
For these reasons, these have often been used to only target physical elements of the urban environment, such as landmarks and street paths.
%
We envision that these could be coupled with techniques for pattern mining, such as the ones cited above, to provide thematic data-based occlusion handling and navigation.
%
This will help users reduce the burden of excessive interaction to focus on spatial patterns while preserving the perception of the spatial context and facilitating tasks that straddle multiple scopes (\textbf{T3} and \textbf{T4}).

\highlight{Moreover, surveyed works use standard techniques in which the users have direct control over the navigation process. A promising avenue for future research involves the exploration of sketch-based navigation coupled with analytics within an urban environment. This could involve, for example, an investigating of the applicability of Hagedorn and D\"{o}llner's sketch-based navigation~\cite{hagedorn_sketch_2008} or Danyluk et al.'s recent proposal~\cite{danyluk_look_2019} for the analysis of data within 3D urban environments.}

\subsection{Empirical validation of visual designs}

While many 3D urban visual analytics systems have been proposed, few empirical studies were done in these scenarios to evaluate the visualizations and interactions proposed (see Section~\ref{sec:how-evaluation}).
%
As discussed throughout this survey, the 3D urban environment adds a great deal of complexity to the navigation, interactions, and occlusion handling. 
%
While some evaluations were done in each of these cases, they are often explored in isolation~\cite{chen_urbanrama_2022}. 
%
This means that understanding how effective these techniques will be for data analytics is largely an open problem.  
%
Furthermore, as seen in Section~\ref{sec:paper_types}, the vast majority of the works concentrate on the development of the systems and on the application domain and not on the evaluation of the visual designs used.
%
This is especially critical when considering the inclusivity and accessibility requirements of various user groups. Creating inclusive visual analytics systems calls for recognizing and addressing the unique challenges faced by individuals with varying abilities (e.g., visual impairments) that may result in considerations of alternative modes of presentation, visualization, navigation, and interaction.
%
As a result of this, the visualization metaphors and interactions used are, in many cases, done without clear guidance~\cite{neuville_3d_2019} or, at best, based on principles and studies done in 2D scenarios. 

However, not all the observations concerning effective visualization designs done in the 2D spatial case can be carried over into the 3D environment~\cite{mota_comparison_2022}.
%
Therefore, there exists a large number of opportunities to assess the current approaches and set the foundations that will guide the design of 3D urban visual analytics systems. In particular, we would like to highlight the great number of opportunities for evaluations concerning the use of visual metaphors and guided explorations described above. 
%
Furthermore, another important aspect that should be further explored is the interplay between occlusion handling techniques and data analytics.
%
In fact, strategies like ghosting and deformation are good examples of techniques that fight occlusion by changing visual elements (e.g., shape, position, or transparency) of the physical elements of the scene.
%
However, these visual elements are often used to depict thematic data (e.g., color, area). 
%
There is a need to understand what is the impact of the use of such techniques on the overall analytics of thematic data and in which situations each technique is most appropriate.
%
Finally, many applications, especially the ones focusing on immersive experiences, try to achieve this via rendering realism.
%
However, similar to the discussion above, the presence of rendering realism (shading, shadows) might interfere with the perception of thematic information.
%
Again, studying the user's perception in such cases is an interesting direction for future research.

\subsection{Open 3D urban visual analytics}

% Our comprehensive review of previous works allow us to derive a series of takeaways for visualization researchers. 
%
As we reviewed and categorized papers, our immediate finding was that, while urban visualization in general has made significant advancements in previous years, there is still a notable gap between visualization contributions and domain requirements.
%
The status quo is one where visualization contributions using 3D urban data are, more often than not, systems that are rarely used beyond the scope of the collaboration that motivated the project in the first place.
%
In the absence of easy-to-use tools designed with visualization best practices in mind, domain experts resort to using an amalgamation of general tools and libraries, from computational notebooks (e.g., Jupyter Notebooks) to comprehensive GIS tools (e.g., ArcGIS)~\cite{yap_free_2022}.
%
While this approach might be sufficient to tackle well-defined urban problems in selected regions, the unprecedented challenges facing cities today call for tools and systems that lower the barrier to performing analyses that are reproducible, replicable, and extensible to enable transdisciplinary and convergent research~\cite{ramaswami_sustainable_2018,lobo_convergence_2021}.
%
Moreover, GIS tools do not consider recent design and evaluation studies and do not provide ways to integrate novel techniques found in visualization studies, hence primarily relying on standard visualization encodings.
%
If done right, visualization and visual analytics can play a key role in creating the needed collaborative environments that can be translated to different regions and use cases.
%
To achieve this, there is a need for (1) community building activities that bring together urban experts and visualization researchers, and (2) the adoption of open-source practices by visualization researchers.

To bring together different communities, we believe that the roadmap outlined by Lan et al.~\cite{lan_visualization_2021} for astrophysics might be appropriate for the urban domain. This path involves joint workshops between visualization researchers and urban experts to be held at conferences in the respective areas, such as IEEE VIS and SimAUD.
%
Examples that can serve as a guideline include ASSETS' UrbanAccess~\cite{froehlich_future_2022}, and VIS' CityVis~\cite{goodwin_unravelling_2021} and EnergyVis workshops.
%
Another potential activity is the creation of visualization challenges using 3D urban data created by experts.

Regarding the adoption of open-source practices, in our survey, none of the visualization contributions were made publicly available, let alone built a community of contributors. In a recent survey by Yap et al.~\cite{yap_free_2022}, out of 70 open-source tools for urban analytics, only one came from the visualization community~\cite{miranda_urban_2017}, and it did not take into account 3D urban data.
%
Adjacent urban topics can provide inspiring examples to the visualization community on how to build and sustain open urban tools. Specifically, OSMnx is a widely used Python-based tool for street network analysis~\cite{boeing_right_2020}. The visualization community should consider that it is not enough to build tools, but that the scientific community should strive for public \emph{reusable} tools and workflows.
%
3D urban visual analytics, much like urban analytics in general, is inherently complex, as the data is oftentimes large, interactions are difficult (especially in 3D), and studies are hard to translate to other regions. While reusability does not seem to be at the forefront of initiatives in the visualization community, well-engineered open efforts, accompanied by outreach efforts, are poised to be embraced by urban experts, given the variability of use cases, data, and tasks. Providing the necessary code base to facilitate urban projects in this domain can lead to not only important domain contributions but also to efforts that provide a more grounded understanding of how experts analyze and visualize 3D urban data.

\subsection{Collaborative urban analytics platforms}

The process of enabling collaborative urban planning and assessment is pivotal for facilitating effective decision- and policy-making, while also encouraging active community involvement in the urban development processes. However, a limited number of existing urban analytics systems provide a platform for multiple stakeholders to collectively visualize, interact with, and contribute to proposed urban developments and policies. Even among the existing systems that do facilitate such collaboration, the emphasis is often placed on tailoring visualization and interaction features primarily for domain experts and practitioners, with less attention being given to incorporating the requirements of the broader public. However, there is a growing need to integrate these systems into a more inclusive context that caters to the diverse technological skills and information needs of diverse individuals. This will help bridge the gap between expert-driven functionalities and the broader public's participation and will lead to the democratization of urban exploration and planning.

% \subsubsection{Development of Systems}

% \begin{itemize}
%     \item should we mention difficulties in the implementation?
%     \item many libraries exist, but often are hard to customize
%     \item Deck.gl, three.gl, ArcGIS
% \end{itemize}

% %
% In planning for future developments, modeling techniques often involve 
% %
% In such cases, the portion of the design space of possible visual representations explored by previous works is far smaller than what has been done in the 2D case.
% %
% There is a strong need for representations
% %

% Urban analyses of 3D environments involve the assessment of the current state of a city 

% As data acquisition technologies and domain analysis get more sophisticated, new challenges ara

% novel visualization metaphors will be needed to represent thematic dimensions.  

% In general, 3D urban analytics applications involve analyzing the current state of a portion of a city


% \subsection{SCRATCH}


% \begin{itemize}
%     \item novel applications
%     \item generalization for multivariate, temporal
%     \item guided explorations: generalizations of 2D approaches
%     \item more concrete link between analytics, navigation and occlusion
%     \item complex network analyses
%     \item lack of design studies    
% \end{itemize}

==> 99-bios.tex <==
\noindent \textbf{Fabio Miranda} is an Assistant Professor in the Dept. of Computer Science at UIC. He received the Ph.D. degree in Computer Science from NYU. His research focuses on large scale data analysis, data structures, and urban data visualization.

\noindent \textbf{Thomas Ortner} is Head of the Geospatial Visualization, Semantic Modelling, and Acquisition group at VRVis. He received the Ph.D. degree from TU Wien in 2021. His research focuses on the combination of visual analytics and real-time rendering.

\noindent \textbf{Maryam Hosseini} is a Postdoctoral associate at the City Form Lab at MIT. She received the Ph.D. in Urban Systems from Rutgers University, and was a research associate at New York University. She works in the intersection between visualization, computer vision and urban science.

\noindent \textbf{Gustavo Moreira} is a PhD student in the Dept. of Computer Science at UIC. He is interested in the intersection between visualization, visual analytics and computer graphics.

\noindent \textbf{Filip Biljecki} is an Assistant Professor at NUS and the principal investigator of the NUS Urban Analytics Lab. He holds an M.Sc. in Geomatics and a Ph.D. in 3D GIS from TU Delft.

\noindent \textbf{Claudio T. Silva} is an Institute Professor of Computer Science at NYU. His research is in the intersection of visualization, data analysis, and geometric computing.

\noindent \textbf{Marcos Lage} is an Associate Professor in the Dept. of Computer Science at UFF.  His  research interests  include  visual  computing, geometry processing, and topological data structures.

\noindent \textbf{Nivan Ferreira} is an Assistant Professor at UFPE. He received his Ph.D. in Computer Science from NYU. His research focuses on interactive data visualization, in particular systems and techniques for analysis spatiotemporal datasets.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> old/urban-3D-sketch.tex <==





\vspace{-0.3cm}
\subsection{Primary Dimensions}

\noindent\textbf{\underline{C1. Paper type.}}
%
We follow Munzner's paper types~\cite{munzner2008process}, with the addition of new data and analysis types to account for domain papers. Papers were classified into: \textbf{system} (papers describing commercial or open-source frameworks)~\cite{ferreira2015urbane,ANG2022103534},
\textbf{technique} (papers describing novel visualization techniques)~\cite{ying2019distortion,https://doi.org/10.1111/cgf.13669},
\textbf{evaluation} (papers evaluating a visualization technique)~\cite{9904453,wang2017users},
\textbf{data} (papers primarily focused on the generation or acquisition of 3D urban data, either through sensing, modeling or simulation)~\cite{BILJECKI2022101809},
\textbf{analysis} (papers primarily focused on the analysis of 3D urban data)~\cite{miranda2018shadow}.

\noindent \textbf{\underline{C2. Use case.}}
%
Papers were classified according to the following primary use cases:
%
\textbf{sunlight access} (assessment of sunlight access or shadow analysis)~\cite{miranda2018shadow,wen2022fast},
\textbf{wind \& ventilation} (assessment of wind or ventilation in urban spaces)~\cite{avini2019wind},
\textbf{view impact} (view to landmarks, green spaces or other urban features)~\cite{yasumoto2011use,yu2016view},
\textbf{energy} (energy consumption, including building energy models)~\cite{gros2014cool,amado2016energy},
\textbf{damage \& disaster management} (assessment of the built environment infrastructure after disasters or extreme weather events)~\cite{vetrivel2015identification,aly2017retrofitting},
\textbf{climate} (interaction between climate or weather and the built environment)~\cite{koch2018compact, mirzaei2021cfd},
\textbf{sound} (interaction between noise and the built environment)~\cite{VANRENTERGHEM2020102362},
\textbf{property cadastre} (assessment of cadastre, including its change over time)~\cite{SHOJAEI201339,wang2017users}.

\vspace{-0.3cm}
\subsection{Data Analysis Dimensions}

\noindent \textbf{\underline{C3. Physical aspect.}}
%
We classify papers according to their main urban physical aspect of focus:
\textbf{buildings} (assessment of building-related data)~\cite{trepci2020effect},
\textbf{streets} (assessment of street-level data)~\cite{yin2017street}, and
\textbf{nature} (study of elements such as parks, trees, rivers, hills in urban environments)~\cite{li20203}.



\noindent \textbf{\underline{C4. Static or dynamic analysis.}}
%
In this category, papers were classified on whether they only support \textbf{static analyses} (i.e., primarily relying on static data)~\cite{HADAVI2021102740}, or \textbf{dynamic analyses} (i.e., enabling the analysis of what-if scenarios following the modification of the built environment)~\cite{miranda2018shadow}.


\noindent \textbf{\underline{C4. Analysis task.}}
We have identified three data analysis tasks in our literature review: 
\textbf{data exploration} (papers describing systems or techniques where the user explores the data in an unstructured fashion for patterns of interest)~\cite{gautier2020co, pasewaldt2013multi}, \textbf{data comparison} (papers where the main analytical task is comparing different datasets or slices of the data)~\cite{NAGPAL2018103}, \textbf{feature identification} (papers where the user is assisted in the identification of features or patterns of interest).

% Elementary: \textbf{lookup tasks}, \textbf{comparison tasks}, \textbf{relation-seeking tasks}
% \textbf{pattern identification}, \textbf{pattern comparison}, \textbf{}

% \begin{itemize}
    % \item Identify
    % \item Explore
% \end{itemize}

\noindent \textbf{\underline{C5. Analysis scope.}}
We have identified four broad analysis scope in our literature review: \textbf{site} (papers that focus on the analysis of an individual site)~\cite{li20193d}, \textbf{single block} (analysis covering a city block)~\cite{zhang2013study}, \textbf{multi-block} (analysis of a region covering multiple blocks)~\cite{heidarinejad2016influence}, \textbf{city} (city-wide analysis)~\cite{li2015xearth}.


\noindent \textbf{\underline{C6. Data resolution \& attributes.}}
In this category, we organized papers depending on how the physical aspect of the data is represented: 
%
\textbf{uniform discretization} (e.g., grid~\cite{KAYNAK2018134,LI2022104505}),
%
\textbf{structural subdivision} (i.e., based on discretization of the physical aspect into smaller units with semantic meaning, e.g., buildings into floors~\cite{NAGPAL2018103} or  massings~\cite{doi:10.1080/13658816.2019.1606431}),
\textbf{structural aggregation} (i.e., based on geographical groupings, e.g., neighborhoods, zip codes);
%
% to the resolution of the data that they use or generate:
%
% \textbf{grid}~\cite{KAYNAK2018134,LI2022104505},
% \textbf{floor}
% ~\cite{NAGPAL2018103}, \textbf{massing}~\cite{doi:10.1080/13658816.2019.1606431}, \textbf{neighborhood}; 
%
and attribute: \textbf{univariate} (considers one target variable), \textbf{multivariate}
(data with more than one attribute)~\cite{10.1145/2816795.2818134}, \textbf{temporal} (data values change over time)~\cite{krietemeyer2019method}.


\vspace{-0.5cm}
\subsection{Visualization \& Interaction Dimension}

\noindent \textbf{\underline{C7. Modality.}}
%
We have identified systems, tools and techniques specifically designed for immersive environments (\textbf{VR}, \textbf{CAVE})~\cite{ZHANG2021128}, \textbf{mobile devices},  \textbf{desktops}~\cite{6280550}.

\noindent \textbf{\underline{C8. Visualization technique.}}
%
This category is based on the visualization techniques employed for the visualization of 3D urban data. In our literature review, we have identifier papers that use \textbf{linked view}~\cite{info13010007}, \textbf{juxtaposed view}~\cite{7390069}, \textbf{embedded view}~\cite{9904453}, \textbf{parallel coordinates}~\cite{8474512}, \textbf{glyphs}~\cite{7390069}, \textbf{streamlines}~\cite{HADAVI2021102740}.

\noindent \textbf{\underline{C9. Navigation technique.}}
%
We classified papers considering the travel aspect of navigation, following Laviola et al.'s taxonomy~\cite{laviola20173d}. We classified papers in the following categories: \textbf{walking}, \textbf{steering}~\cite{CHASSIN2022104432}, \textbf{selection-based travel}~\cite{ZHANG2021128} (including \textbf{target-based} and \textbf{route-planning travel}), \textbf{manipulation-based travel}~\cite{9495135} (including \textbf{viewpoint manipulation} and \textbf{world manipulation}).
%
% For wayfinding, we considered the following cues or aids: \textbf{user-centered wayfinding cues} and \textbf{environment-centered wayfinding cues}.

\vspace{-0.5cm}


% \begin{itemize}
%     \item Scale
%     \item Data interoperability
%     \item Burden of 3D interactions
%     \item Guidance
%     \item Multidimensional visualization
%     \item Collaborative environments
% \end{itemize}


%-------------------------------------------------------------------------


% biblatex with biber
% \printbibliography                

\clearpage
\noindent \textbf{Short Biographies}

\noindent \textbf{Fabio Miranda} is an Assistant Professor in the Computer Science Dept. at University of Illinois at Chicago. He received the Ph.D. degree in computer science from New York University and the M.Sc. degree in computer science from PUC-Rio. His research focuses on large scale data analysis, data structures, and urban data visualization.

\noindent \textbf{Thomas Ortner} is Head of the `Geospatial Visualization, Semantic Modelling, and Acquisition' group at VRVis. He received his degree in `Computer Graphics Programming' from the Faculty of Science and Engineering at the University of Hull (UK) in 2008. Thomas Ortner already worked as a software engineer and researcher for several years and completed his PhD at TU Wien in in 2021. His PhD research concerns the combination of the two worlds of visual analytics and real-time rendering.

%is a Group Lead and Researcher at VRVis in Vienna. He received the Ph.D. degree in computer science from TU Wien. His research interests include 3D geospatial rendering, visual analytics, and integration of 3D geometric and attribute data.

\noindent \textbf{Maryam Hosseini} is a Postdoctoral associate at the City Form Lab at MIT. She received the Ph.D. in urban systems from Rutgers University, and was a research associate at New York University. She works in the intersection between visualization, computer vision and urban science. She is especially interested in tackling urban accessibility problems through the novel use of computer vision and visualization techniques.

\noindent \textbf{Gustavo Moreira} is a PhD student in the Computer Science Dept. at University of Illinois at Chicago. He is interested in the intersection between visualization, visual analytics and computer graphics.

\noindent \textbf{Marcos Lage} is an Associate Professor in the Dept. of Computer Science at Universidade Federal Fluminense in Brazil, and is one of the principal investigators  of  the  Prograf  Lab.  His  research interests  include  aspects  of  visual  computing, especially scientific and information visualization, geometry processing, and topological data structures. He has a Ph.D. in applied mathematics from PUC-Rio.

\noindent \textbf{Filip Biljecki} is an Assistant Professor at the National University of Singapore and the principal investigator of the NUS Urban Analytics Lab.
He holds an M.Sc. in Geomatics and a Ph.D. in 3D GIS from the Delft University of Technology in the Netherlands.

\noindent \textbf{Claudio T. Silva} is an Institute Professor of Computer Science and Engineering at NYU Tandon School of Engineering, and Professor of Data Science at NYU. His research lies in the intersection of visualization, data analysis, and geometric computing, and recently has focused on urban and sports data. He has received a number of awards: IEEE Fellow, IEEE Visualization Technical Achievement Award, and elected chair of the IEEE Visualization \& Graphics Technical Committee.

    \noindent \textbf{Nivan Ferreira} is an Assistant Professor at Centro de Informática at Universidade Federal de Pernambuco in Brazil. He received his Ph.D. in Computer Science from New York University. His research focuses on many aspects of interactive data visualization, in particular systems and techniques for analysis spatiotemporal datasets.


